ITBench: Evaluating AI Agents across Diverse Real-World IT Automation Tasks

Realizing the vision of using AI agents to automate critical IT tasks depends on the ability to measure and understand effectiveness of proposed solutions. We introduce ITBench, a framework that offers a systematic methodology for benchmarking AI agents to address real-world IT automation tasks. Our initial release targets three key areas: Site Reliability Engineering (SRE), Compliance and Security Operations (CISO), and Financial Operations (FinOps). The design enables AI researchers to understand the challenges and opportunities of AI agents for IT automation with push-button workflows and interpretable metrics. ITBench includes an initial set of 94 real-world scenarios, which can be easily extended by community contributions. Our results show that agents powered by state-of-the-art models resolve only 13.8% of SRE scenarios, 25.2% of CISO scenarios, and 0% of FinOps scenarios. We expect ITBench to be a key enabler of AI-driven IT automation that is correct, safe, and fast.

==> colorboxdefs.tex <==
\newtcolorbox{observationbox}[1][]{
        colback=envfill,
        colbacktitle=envfill,
        colframe=envborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Observation \hfill #1},
        rounded corners,
        toptitle=0.7mm,
        bottomtitle=0.7mm
}
\newtcolorbox{goldpatchbox}[1][]{
        colback=goldpatchfill,
        colbacktitle=goldpatchfill,
        colframe=goldpatchborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Gold Patch \hfill #1},
        rounded corners,
        toptitle=0.7mm,
        bottomtitle=0.7mm
}
\newtcolorbox{issuebox}[1][]{
        colback=issuefill,
        colbacktitle=issuefill,
        colframe=issueborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Issue \hfill #1},
        rounded corners,
        toptitle=1mm
}

\newtcolorbox{fileviewerbox}[1]{
        enhanced,
        breakable,
        boxrule = 1.5pt,
        fontupper = \small,
        fonttitle = \bf\color{black},
        arc = 5pt,
        rounded corners,
        colframe = black,
        colbacktitle = srecream,
        colback = srecream,
        title = #1,
        left=4pt % moves left over a bit to make text never overlaps with border
}


\newtcolorbox{toolbox}[1][]{
    enhanced,
    breakable,
    boxrule=1pt,
    fontupper=\small,
    fonttitle=\bfseries\color{black},
    arc=3pt,
    rounded corners,
    colframe=black,
    colbacktitle=swecream,
    colback=swecream,
    title={Action \hfill #1},
    left=2mm,
    right=2mm,
    top=1mm,
    bottom=1mm
}
\newtcolorbox{alertclearbox}[1][]{
        colback=goldpatchfill,
        colbacktitle=goldpatchfill,
        colframe=goldpatchborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Alert Cleared \hfill #1},
        rounded corners,
        toptitle=0.7mm,
        bottomtitle=0.7mm
}
\newtcolorbox{alertbox}[1][]{
        colback=issuefill,
        colbacktitle=issuefill,
        colframe=issueborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Alert \hfill #1},
        rounded corners,
        toptitle=1mm
}
\newtcolorbox{actionbox}[1][]{
    enhanced,
    breakable,
    boxrule=1pt,
    fontupper=\small,
    fonttitle=\bfseries\color{black},
    arc=3pt,
    rounded corners,
    colframe=black,
    colbacktitle=swecream,
    colback=swecream,
    title={Action \hfill #1},
    left=2mm,
    right=2mm,
    top=1mm,
    bottom=1mm
}
\newtcolorbox{thoughtbox}[1][]{
        colback=agentfill,
        colbacktitle=agentfill,
        colframe=agentborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Thought \hfill #1},
        rounded corners,
        toptitle=1mm,
        lower separated=false
}

\newtcolorbox{keyinsightbox}[1][]{
        colback=envfill,
        colbacktitle=envfill,
        colframe=envborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Key insights -- #1},
        rounded corners,
        toptitle=0.2mm,
        bottomtitle=0.2mm
}

\newtcolorbox{jsonbox}[1][]{
        colback=envfill,
        colbacktitle=envfill,
        colframe=envborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\textwidth,
        breakable,
        enhanced,
        before=\noindent, % Prevent indentation before the box
        after=\vspace{0mm}, % Remove extra space after the box
        frame hidden, % Prevent redrawing the frame after a break
        % interior hidden, % Prevent double interior filling
        title={#1},
        rounded corners,
        toptitle=0.7mm,
        bottomtitle=0.7mm
}


% Additional Color box for CISO-agent
\newtcolorbox{taskfinishedbox}[1][]{
        colback=goldpatchfill,
        colbacktitle=goldpatchfill,
        colframe=goldpatchborder,
        arc=5pt,
        fontupper=\small,
        fonttitle=\bfseries\color{black},
        boxrule=0.5mm,
        boxsep=1mm,
        width=\linewidth,
        breakable,
        title={Task Finished \hfill #1},
        rounded corners,
        toptitle=0.7mm,
        bottomtitle=0.7mm
}

% \newtcolorbox{jsonbox*}[1][]{
%         colback=envfill,
%         colbacktitle=envfill,
%         colframe=envborder,
%         arc=5pt,
%         fontupper=\small,
%         fonttitle=\bfseries\color{black},
%         boxrule=0.5mm,
%         boxsep=1mm,
%         width=\textwidth, % Full width of the page
%         breakable,
%         title={#1},
%         rounded corners,
%         toptitle=0.7mm,
%         bottomtitle=0.7mm,
%         enlarge left by=0mm,
%         enlarge right by=0mm
% }
\lstdefinelanguage{json}{
    basicstyle=\linespread{1.1}\footnotesize\ttfamily,
    breaklines=true, % Enable line wrapping
    showstringspaces=false,
    string=[s]{"}{"},
    stringstyle=\color{black},
    comment=[l]{//},
    commentstyle=\color{gray},
    keywordstyle=\color{green!40!black},
    moredelim=[b][\color{black}]{\{}
}
